An upper bound on the denominator of Eisenstein classes in Bianchi manifolds

A general conjecture of Harder relates the denominator of the Eisenstein cohomology of certain locally symmetric spaces to special values of $L$-functions. In this paper we consider the locally symmetric space $\operatorname{SL}_2(\mathcal{O}) \backslash \mathbb{H}_3$ where $\mathcal{O}$ is the ring of integers of an imaginary quadratic field $K$ and $\mathbb{H}_3$ is the hyperbolic $3$-space. Tobias Berger proves a lower bound on the denominator of the Eisenstein cohomology in certain cases. The goal of this paper is to show how results of Ito and Sczech can be used to prove an upper bound on the denominator in terms of a special value of a Hecke $L$-function. When the class number of $K$ is one, we combine this result with Berger's result to obtain the exact denominator.

==> todo.tex <==
\section{todo}
\begin{enumerate}
\item Include Pierre's comments: the table of explicit denominators, the description of the paths and maybe redo figures? Add him in aknowledgment. When h=1 remove congruence of D!
\item Sheng-Chi Shih: the characters are not on class groups, state corollary if terms of congruence ideals
\end{enumerate}

